Revealing the Self: Brainwave-Based Human Trait Identification

People exhibit unique emotional responses. In the same scenario, the emotional reactions of two individuals can be either similar or vastly different. For instance, consider one person's reaction to an invitation to smoke versus another person's response to a query about their sleep quality. The identification of these individual traits through the observation of common physical parameters opens the door to a wide range of applications, including psychological analysis, criminology, disease prediction, addiction control, and more. While there has been previous research in the fields of psychometrics, inertial sensors, computer vision, and audio analysis, this paper introduces a novel technique for identifying human traits in real time using brainwave data. To achieve this, we begin with an extensive study of brainwave data collected from 80 participants using a portable EEG headset. We also conduct a statistical analysis of the collected data utilizing box plots. Our analysis uncovers several new insights, leading us to a groundbreaking unified approach for identifying diverse human traits by leveraging machine learning techniques on EEG data. Our analysis demonstrates that this proposed solution achieves high accuracy. Moreover, we explore two deep-learning models to compare the performance of our solution. Consequently, we have developed an integrated, real-time trait identification solution using EEG data, based on the insights from our analysis. To validate our approach, we conducted a rigorous user evaluation with an additional 20 participants. The outcomes of this evaluation illustrate both high accuracy and favorable user ratings, emphasizing the robust potential of our proposed method to serve as a versatile solution for human trait identification.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> table-auto-weka.tex <==
\begin{table*}[!ht]
    \centering
    \small
    \caption{Machine Learning Models from Auto-WEKA package}
    \begin{tabular}{|l|c|c|}
        \hline
        \textbf{\begin{tabular}[c]{@{}l@{}}Predicted Trait \\ - Emotion\end{tabular}} & \textbf{Classifier} & \textbf{\begin{tabular}[c]{@{}c@{}}Accuracy \\ (\%)\end{tabular}} \\ \hline
        Smoker - Happy & LWL & 70.67 \\ \hline
        Smoker - Meditation & Random Tree & 59.21 \\ \hline
        Smoker - Neutral & J48 & 65.28 \\ \hline
        Smoker - Sad & JRip & 71.05 \\ \hline
        Alcoholic - Happy & Naïve Bayes & 62.67 \\ \hline
        Alcoholic - Meditation & \begin{tabular}[c]{@{}c@{}}Naïve Bayes \\ Multinomial\end{tabular} & 61.84 \\ \hline
        Alcoholic - Neutral & Simple Logistic & 65.28 \\ \hline
        Alcoholic - Sad & AdaBoost M1 & 67.11 \\ \hline
        Believer - Happy & Voted Perceptron & 89.33 \\ \hline
        Believer - Meditation & Voted Perceptron & 89.47 \\ \hline
        Believer - Neutral & SMO & 90.28 \\ \hline
        Believer - Sad & OneR & 93.42 \\ \hline
        Practitioner - Happy & AdaBoost M1 & 76.32 \\ \hline
        Practitioner - Meditation & J48 & 77.63 \\ \hline
        Practitioner - Neutral & J48 & 44.44 \\ \hline
        Practitioner - Sad & Bagging & 76.35 \\ \hline
        Exercise - Happy & Bagging & 82.67 \\ \hline
        Exercise - Meditation & PART & 81.58 \\ \hline
        Exercise - Neutral & OneR & 90.28 \\ \hline
        Exercise - Sad & Vote & 82.89 \\ \hline
        Fast food - Happy & Simple Logistic & 46.67 \\ \hline
        Fast food - Meditation & Decision Stump & 51.32 \\ \hline
        Fast food - Neutral & Bagging & 47.22 \\ \hline
        Fast food - Sad & LWL & 63.16 \\ \hline
        Fat - Happy & Bagging & 50.67 \\ \hline
        Fat - Meditation & Decision Stump & 65.79 \\ \hline
        Fat - Neutral & \begin{tabular}[c]{@{}c@{}}Attribute Selected \\ Classifier\end{tabular} & 55.56 \\ \hline
        Fat - Sad & Multilayer Perceptron & 59.21 \\ \hline
        \end{tabular}
        \begin{tabular}{|l|c|c|}
        \hline
        \textbf{\begin{tabular}[c]{@{}l@{}}Predicted Trait \\ - Emotion\end{tabular}} & \textbf{Classifier} & \textbf{\begin{tabular}[c]{@{}c@{}}Accuracy \\ (\%)\end{tabular}} \\ \hline
        Sugar - Happy & SMO & 62.67 \\ \hline
        Sugar - Meditation & SMO & 63.16 \\ \hline
        Sugar - Neutral & \begin{tabular}[c]{@{}c@{}}Random \\ Sub Space\end{tabular} & 63.89 \\ \hline
        Sugar - Sad & SMO & 65.79 \\ \hline
        Vegetable - Happy & Logistic & 70.67 \\ \hline
        Vegetable - Meditation & Logistic & 72.37 \\ \hline
        Vegetable - Neutral & \begin{tabular}[c]{@{}c@{}}Multilayer \\ Perceptron\end{tabular} & 79.17 \\ \hline
        Vegetable - Sad & J48 & 76.32 \\ \hline
        Sleep time - Happy & BayesNet & 54.67 \\ \hline
        Sleep time - Meditation & Decision Stump & 53.95 \\ \hline
        Sleep time - Neutral & Decision Stump & 52.78 \\ \hline
        Sleep time - Sad & REPTree & 53.95 \\ \hline
        Sleeping Problem - Happy & REPTree & 58.67 \\ \hline
        Sleeping Problem - Meditation & JRip & 46.05 \\ \hline
        Sleeping Problem - Neutral & Bagging & 44.44 \\ \hline
        Sleeping Problem - Sad & Decision Stump & 53.95 \\ \hline
        Heart disease- Happy & PART & 76.00 \\ \hline
        Heart disease- Meditation & J48 & 81.58 \\ \hline
        Heart disease - Neutral & PART & 75.00 \\ \hline
        Heart disease - Sad & Decision Stump & 77.63 \\ \hline
        Diabetes - Happy & Bagging & 60.00 \\ \hline
        Diabetes - Meditation & Decision Table & 59.21 \\ \hline
        Diabetes - Neutral & LWL & 94.44 \\ \hline
        Diabetes - Sad & Bagging & 65.79 \\ \hline
        Stroke - Happy & Decision Stump & 57.33 \\ \hline
        Stroke - Meditation & IBk & 92.11 \\ \hline
        Stroke - Neutral & LWL & 69.44 \\ \hline
        Stroke - Sad & Decision Stump & 56.58 \\ \hline
        \end{tabular}
    \label{table1}
\end{table*}

==> table-config-dl-moodels.tex <==
\begin{table}[!ht]
\small
\centering
\caption{Configuration of the Deep Learning Models}
\label{tab:table_lstm}
\begin{tabular} {|p{1.5in} | p{1.35in} |}
   \hline
\textbf{ Deep Learning Layer } & \textbf{ Value}\\ \hline
LSTM Layer & 50 hidden units\\ \hline
BiLSTM Layer & 50 hidden units\\ \hline
Dropout Layer & 20\% dropout Layer\\ \hline
Fully Connected Layer & 1 Fully Connected Layer\\ \hline
Classification Layer & SoftMax\\ \hline
Loss Function & Categorical Cross-Entropy\\ \hline
ADAM & - \\ \hline
No. of Epochs & 50 \\ \hline
Batch Size & 32 \\ \hline
Initial Learning Rate & 0.001 \\  \hline 
\end{tabular}
\end{table}

==> table-lstm-bilstm.tex <==
\begin{table*}[!ht]
\small
    \centering
    % \small
    \caption{Deep Learning Models}
    \begin{tabular}{|l|cc|}
        \hline
        \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Predicted Trait \\ - Emotion\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Accuracy (\%)}} \\ \cline{2-3} 
         & \multicolumn{1}{l|}{\textbf{LSTM}} & \multicolumn{1}{l|}{\textbf{BiLSTM}} \\ \hline
        Smoker - Happy & \multicolumn{1}{c|}{69.23} & 61.54 \\ \hline
        Smoker - Meditation & \multicolumn{1}{c|}{46.15} & 38.46 \\ \hline
        Smoker - Neutral & \multicolumn{1}{c|}{50.00} & 66.67 \\ \hline
        Smoker - Sad & \multicolumn{1}{c|}{42.86} & 35.71 \\ \hline
        Alcoholic - Happy & \multicolumn{1}{c|}{61.54} & 53.85 \\ \hline
        Alcoholic - Meditation & \multicolumn{1}{c|}{53.85} & 46.15 \\ \hline
        Alcoholic - Neutral & \multicolumn{1}{c|}{66.67} & 58.33 \\ \hline
        Alcoholic - Sad & \multicolumn{1}{c|}{42.86} & 35.71 \\ \hline
        Believer - Happy & \multicolumn{1}{c|}{92.31} & 69.23 \\ \hline
        Believer - Meditation & \multicolumn{1}{c|}{84.62} & 76.92 \\ \hline
        Believer - Neutral & \multicolumn{1}{c|}{75.00} & 91.67 \\ \hline
        Believer - Sad & \multicolumn{1}{c|}{78.57} & 71.43 \\ \hline
        Practitioner - Happy & \multicolumn{1}{c|}{53.85} & 30.77 \\ \hline
        Practitioner - Meditation & \multicolumn{1}{c|}{53.85} & 46.15 \\ \hline
        Practitioner - Neutral & \multicolumn{1}{c|}{41.67} & 41.67 \\ \hline
        Practitioner - Sad & \multicolumn{1}{c|}{42.86} & 35.71 \\ \hline
        Exercise - Happy & \multicolumn{1}{c|}{92.31} & 92.31 \\ \hline
        Exercise - Meditation & \multicolumn{1}{c|}{84.62} & 92.31 \\ \hline
        Exercise - Neutral & \multicolumn{1}{c|}{75.00} & 83.33 \\ \hline
        Exercise - Sad & \multicolumn{1}{c|}{64.29} & 78.57 \\ \hline
        Fast food - Happy & \multicolumn{1}{c|}{46.15} & 46.15 \\ \hline
        Fast food - Meditation & \multicolumn{1}{c|}{69.23} & 38.46 \\ \hline
        Fast food - Neutral & \multicolumn{1}{c|}{50.00} & 41.67 \\ \hline
        Fast food - Sad & \multicolumn{1}{c|}{57.14} & 35.71 \\ \hline
        Fat - Happy & \multicolumn{1}{c|}{46.15} & 46.15 \\ \hline
        Fat - Meditation & \multicolumn{1}{c|}{61.54} & 46.15 \\ \hline
        Fat - Neutral & \multicolumn{1}{c|}{50.00} & 41.67 \\ \hline
        Fat - Sad & \multicolumn{1}{c|}{71.43} & 78.57 \\ \hline
        \end{tabular}
        \begin{tabular}{|l|cc|}
        \hline
        \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Predicted Trait \\ - Emotion\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Accuracy (\%)}} \\ \cline{2-3} 
         & \multicolumn{1}{l|}{\textbf{LSTM}} & \multicolumn{1}{l|}{\textbf{BiLSTM}} \\ \hline
        Sugar - Happy & \multicolumn{1}{c|}{61.54\%} & 61.54\% \\ \hline
        Sugar - Meditation & \multicolumn{1}{c|}{69.23\%} & 53.85\% \\ \hline
        Sugar - Neutral & \multicolumn{1}{c|}{66.67\%} & 75.00\% \\ \hline
        Sugar - Sad & \multicolumn{1}{c|}{50.00\%} & 57.14\% \\ \hline
        Vegetable - Happy & \multicolumn{1}{c|}{76.92\%} & 84.62\% \\ \hline
        Vegetable - Meditation & \multicolumn{1}{c|}{76.92\%} & 69.23\% \\ \hline
        Vegetable - Neutral & \multicolumn{1}{c|}{58.33\%} & 83.33\% \\ \hline
        Vegetable - Sad & \multicolumn{1}{c|}{71.43\%} & 57.14\% \\ \hline
        Sleep time - Happy & \multicolumn{1}{c|}{69.23\%} & 53.85\% \\ \hline
        Sleep time - Meditation & \multicolumn{1}{c|}{53.85\%} & 38.46\% \\ \hline
        Sleep time - Neutral & \multicolumn{1}{c|}{41.67\%} & 66.67\% \\ \hline
        Sleep time - Sad & \multicolumn{1}{c|}{64.29\%} & 35.71\% \\ \hline
        Sleeping Problem - Happy & \multicolumn{1}{c|}{61.54\%} & 61.54\% \\ \hline
        Sleeping Problem - Meditation & \multicolumn{1}{c|}{46.15\%} & 61.54\% \\ \hline
        Sleeping Problem - Neutral & \multicolumn{1}{c|}{41.67\%} & 25.00\% \\ \hline
        Sleeping Problem - Sad & \multicolumn{1}{c|}{57.14\%} & 42.86\% \\ \hline
        Heart disease - Happy & \multicolumn{1}{c|}{61.54\%} & 76.92\% \\ \hline
        Heart disease - Meditation & \multicolumn{1}{c|}{76.92\%} & 92.31\% \\ \hline
        Heart disease - Neutral & \multicolumn{1}{c|}{83.33\%} & 66.67\% \\ \hline
        Heart disease - Sad & \multicolumn{1}{c|}{64.29\%} & 92.86\% \\ \hline
        Diabetes - Happy & \multicolumn{1}{c|}{69.23\%} & 76.92\% \\ \hline
        Diabetes - Meditation & \multicolumn{1}{c|}{69.23\%} & 69.23\% \\ \hline
        Diabetes - Neutral & \multicolumn{1}{c|}{66.67\%} & 66.67\% \\ \hline
        Diabetes - Sad & \multicolumn{1}{c|}{57.14\%} & 50.00\% \\ \hline
        Stroke - Happy & \multicolumn{1}{c|}{92.31\%} & 76.92\% \\ \hline
        Stroke - Meditation & \multicolumn{1}{c|}{84.62\%} & 92.31\% \\ \hline
        Stroke - Neutral & \multicolumn{1}{c|}{83.33\%} & 83.33\% \\ \hline
        Stroke - Sad & \multicolumn{1}{c|}{100.00\%} & 85.71\% \\ \hline
        \end{tabular}
    \label{table2}
\end{table*}
